MemFuse: Multi-Source Memory Fusion from Fragmented Observations

Long-term memory is essential for agents that operate across extended interactions, yet existing memory systems and benchmarks predominantly focus on single-source textual histories. In realistic settings, however, relevant information is often fragmented across applications and devices, as well as across users and time, requiring agents to integrate dispersed observations into coherent episodic memories while preserving their source provenance. To address these gaps, we introduce **MemFuseBench**, a benchmark for *multi-source memory fusion*. MemFuseBench is built with a Scene-to-Sensor pipeline that synthesizes controllable scenarios into source-tagged observations, evidence-grounded questions, and adversarial distractors. It enables systematic evaluation of temporal reasoning, cross-source evidence fusion, and robustness to noise. We further propose **MemFuse**, a structured memory system that preserves source-level evidence in event-layer atomic memory and organizes related atomic events into cluster-layer fused memory within a causal fusion graph. During retrieval, MemFuse retrieves and organizes related evidence fragments while maintaining traceability to original source events. Experiments on MemFuseBench show that MemFuse achieves the best overall performance among the evaluated memory systems under all three LLM settings and consistently improves performance on questions requiring cross-source evidence fusion.

==> prompt_tex/1e74d81e324aff07118fc8082be81f88.md.tex <==
\markdownRendererDocumentBegin
Generate a retrieval plan for the question below.\markdownRendererInterblockSeparator
{}Question: \markdownRendererLeftBrace{}query\markdownRendererRightBrace{}\linebreak
{}Question time: \markdownRendererLeftBrace{}query\markdownRendererUnderscore{}time\markdownRendererUnderscore{}text\markdownRendererRightBrace{}\linebreak
{}Question weekday/calendar reference: \markdownRendererLeftBrace{}weekday\markdownRendererUnderscore{}calendar\markdownRendererUnderscore{}text\markdownRendererRightBrace{}\linebreak
{}Requester: \markdownRendererLeftBrace{}requester\markdownRendererUnderscore{}id or 'unknown'\markdownRendererRightBrace{}\markdownRendererInterblockSeparator
{}Output JSON schema. The strings below are field descriptions, not default values. Do not copy the description strings; output real JSON values:\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{prompt_tex/3cf4c76dfa10c006256353f7e5205c47.verbatim}{json}\markdownRendererInterblockSeparator
{}Decision rules:\markdownRendererInterblockSeparator
{}\markdownRendererUlBegin
\markdownRendererUlItem query\markdownRendererUnderscore{}rewrite has the highest priority and must not be distorted by later control strategies:\markdownRendererInterblockSeparator
{}\markdownRendererUlBegin
\markdownRendererUlItem Every semantic query must preserve the main answer shape of the original question.\markdownRendererUlItemEnd 
\markdownRendererUlItem Semantic queries should retrieve evidence events, not draft the final answer.\markdownRendererUlItemEnd 
\markdownRendererUlItem If the original question asks for a full sequence, what exactly happened, a timeline, a process, or an experience, semantic\markdownRendererUnderscore{}queries must keep that process-reconstruction intent.\linebreak
{}Do not rewrite it into a why/cause query.\markdownRendererUlItemEnd 
\markdownRendererUlItem Only generate cause-oriented rewrites when the original question explicitly asks why, for the reason, what caused it, or how it happened.\markdownRendererUlItemEnd 
\markdownRendererUlItem The first semantic\markdownRendererUnderscore{}query should stay close to the core wording of the original question.\linebreak
{}Only compress, remove redundancy, and highlight keywords.\markdownRendererUlItemEnd 
\markdownRendererUlItem Later semantic queries should cover complementary evidence facets, such as participant actions, device observations, location/object/state changes, before/after context, or source-specific viewpoints.\linebreak
{}Do not make all rewrites near-duplicates.\markdownRendererUlItemEnd 
\markdownRendererUlItem Preserve detail requests such as colors, quantities, durations, counts, game rounds, health readings, emotional reactions, care/concern, conflicts, viewpoints, and explicit objects.\linebreak
{}These details often decide checklist credit.\markdownRendererUlItemEnd 
\markdownRendererUlItem For contradiction or record-arbitration questions, preserve every competing value and source in both semantic\markdownRendererUnderscore{}queries and bm25\markdownRendererUnderscore{}query.\linebreak
{}Include nearby evidence facets such as timestamps, pulse/score/count/unit fields, manual entry vs automated device source, and transcription/recording context when the original question compares two records.\markdownRendererUlItemEnd 
\markdownRendererUlItem bm25\markdownRendererUnderscore{}query should remain close to the original question and keep exact lexical anchors. Do not replace names/devices/objects with generic paraphrases in bm25\markdownRendererUnderscore{}query.\markdownRendererUlItemEnd 
\markdownRendererUlEnd \markdownRendererUlItemEnd 
\markdownRendererUlItem Set time\markdownRendererUnderscore{}window only when one bounded time span is useful for retrieval. A calendar clue is not enough by itself.\markdownRendererInterblockSeparator
{}\markdownRendererUlBegin
\markdownRendererUlItem Disable time\markdownRendererUnderscore{}window for broad or longitudinal questions spanning multiple days, such as "this week", "past week", "over the week", "eventually", "from X to Y", "lead to ... later", "commitments/plans this week", "everything bought/ordered this week", or questions mentioning multiple distinct dates.\linebreak
{}These need semantic/BM25 coverage across days rather than one day crowding out other evidence.\markdownRendererUlItemEnd 
\markdownRendererUlItem Disable time\markdownRendererUnderscore{}window when the question has no explicit date and the only time clue is a broad period like "this week" or "recently".\markdownRendererUlItemEnd 
\markdownRendererUlItem If a question contains both an initial event date and a later outcome date, do not choose only the initial date.\linebreak
{}Disable time\markdownRendererUnderscore{}window unless the question asks specifically about one bounded episode.\markdownRendererUlItemEnd 
\markdownRendererUlEnd \markdownRendererUlItemEnd 
\markdownRendererUlItem When time\markdownRendererUnderscore{}window.enabled=true, always output both start\markdownRendererUnderscore{}time and end\markdownRendererUnderscore{}time. The retrieval code cannot use a date-only window.\markdownRendererInterblockSeparator
{}\markdownRendererUlBegin
\markdownRendererUlItem For date-only questions such as an explicit calendar date, a named weekday, "that day", "all day", or "throughout the day", use start\markdownRendererUnderscore{}time="00:00:00" and end\markdownRendererUnderscore{}time="23:59:59".\markdownRendererUlItemEnd 
\markdownRendererUlItem Do not treat a question as date-only if it contains a part-of-day or activity/session anchor. Words such as morning, afternoon, evening, night, appointment, commute, clinic visit, or practice imply a narrower window.\markdownRendererUlItemEnd 
\markdownRendererUlItem Do not infer a clock range from meal/session labels alone, such as dinner, breakfast, lunch, movie night, board game session, yoga session, or conversation, unless the question also gives an explicit time, part-of-day, or asks only about that bounded session.\linebreak
{}If the label may be colloquial or the key anchors are topical, prefer semantic/BM25 retrieval with time\markdownRendererUnderscore{}window disabled or with a low quota.\markdownRendererUlItemEnd 
\markdownRendererUlItem Sleep/night questions often refer to evidence recorded around wake-up, not the whole daytime.\linebreak
{}If the question asks about "that night", sleep quality, sleep score, sleep tracker/bed sensor records, or an earlier-morning vs later-morning sleep summary, do not use a full-day daytime window.\linebreak
{}Use the referenced morning window, usually 00:00:00-09:59:59, and rely on exact sleep-score/duration/device anchors for prior-night evidence.\markdownRendererUlItemEnd 
\markdownRendererUlItem When a question names a weekday/date but asks about sleep "that night" or "earlier that morning", the relevant evidence is the early-morning sleep records for that resolved date, not the entire daytime.\linebreak
{}Keep sleep-score numbers, durations, and device names as lexical anchors.\markdownRendererUlItemEnd 
\markdownRendererUlItem Explicit part-of-day words are stronger than a bare calendar date. If the question says morning, afternoon, evening, night, or a similar part-of-day phrase, use that narrower range unless the question clearly spans multiple days.\markdownRendererUlItemEnd 
\markdownRendererUlItem When both a date and a part-of-day/session anchor are present, keep the narrower part-of-day/session window instead of expanding to the full day.\markdownRendererUlItemEnd 
\markdownRendererUlItem Use null start\markdownRendererUnderscore{}time/end\markdownRendererUnderscore{}time only when time\markdownRendererUnderscore{}window.enabled=false.\markdownRendererUlItemEnd 
\markdownRendererUlEnd \markdownRendererUlItemEnd 
\markdownRendererUlItem Relative weekday/date normalization is critical:\markdownRendererInterblockSeparator
{}\markdownRendererUlBegin
\markdownRendererUlItem Use Question time as the reference point for relative dates and weekday names.\markdownRendererUlItemEnd 
\markdownRendererUlItem If the question mentions a weekday such as Monday/Tuesday/Wednesday/Thursday/Friday/Saturday/Sunday without an explicit calendar date, choose the most recent matching weekday at or before Question time.\linebreak
{}Do not choose an arbitrary weekday from the same week.\markdownRendererUlItemEnd 
\markdownRendererUlItem If the weekday in the question is the same weekday as Question time and the question describes an event that could already have happened, use Question time's date.\markdownRendererUlItemEnd 
\markdownRendererUlItem If the question says "last", "yesterday", "earlier", "this morning", "tonight", or similar relative wording, resolve it strictly relative to Question time.\markdownRendererUlItemEnd 
\markdownRendererUlItem If the question names a weekday night and the evidence may continue after midnight, anchor the window to the named weekday and use evening/night hours; do not shift the whole window to the next day.\markdownRendererUlItemEnd 
\markdownRendererUlItem If you cannot confidently resolve a weekday/date from Question time, set confidence below 0.6 rather than inventing a high-confidence date.\markdownRendererUlItemEnd 
\markdownRendererUlEnd \markdownRendererUlItemEnd 
\markdownRendererUlItem Normalize vague times with these ranges; do not expand morning/evening into the whole day:\markdownRendererInterblockSeparator
{}\markdownRendererUlBegin
\markdownRendererUlItem pre-dawn: 00:00:00-05:59:00\markdownRendererUlItemEnd 
\markdownRendererUlItem early morning: 06:00:00-09:59:00\markdownRendererUlItemEnd 
\markdownRendererUlItem morning: 05:00:00-11:59:00\markdownRendererUlItemEnd 
\markdownRendererUlItem noon: 11:00:00-13:59:00\markdownRendererUlItemEnd 
\markdownRendererUlItem afternoon: 13:00:00-17:59:00\markdownRendererUlItemEnd 
\markdownRendererUlItem dusk: 17:00:00-19:59:00\markdownRendererUlItemEnd 
\markdownRendererUlItem evening/night: 18:00:00-23:59:00\markdownRendererUlItemEnd 
\markdownRendererUlItem Enable coverage when the question requires complete coverage across multiple people, devices, places, sources, or viewpoints.\linebreak
{}Examples: comparing parties, explaining each one separately, all related people/device states, who was present, or what each source observed.\linebreak
{}Do not enable coverage for a single subject's cause, state, or fact query.\markdownRendererUlItemEnd 
\markdownRendererUlItem Enable timeline\markdownRendererUnderscore{}mode when the answer needs multiple ordered steps, such as a full sequence, route/itinerary, key milestones, phase changes, repeated attempts, multiple rounds, a morning/day reconstruction, or the process from one time to another.\linebreak
{}Do not enable it for a single-point reason or single fact query.\markdownRendererUlItemEnd 
\markdownRendererUlEnd \markdownRendererUlItemEnd 
\markdownRendererUlItem temporal\markdownRendererUnderscore{}neighbors decision table:\markdownRendererInterblockSeparator
{}\markdownRendererUlBegin
\markdownRendererUlItem Enable when the question explicitly asks for a full sequence, timeline, total occurrences, each occurrence, a continuous period, a before/after progression, dialogue followed by actions, or a multi-step activity where adjacent snippets around hit events are needed in context.\markdownRendererUlItemEnd 
\markdownRendererUlItem Disable for ordinary why/reason/state/existence/how questions.\linebreak
{}Do not enable merely because a question is causal; multi-subject coverage also does not imply temporal\markdownRendererUnderscore{}neighbors.\markdownRendererUlItemEnd 
\markdownRendererUlItem radius defaults to 3.\linebreak
{}Use 1-2 only for very short point-context questions.\markdownRendererUlItemEnd 
\markdownRendererUlEnd \markdownRendererUlItemEnd 
\markdownRendererUlItem seed.time\markdownRendererUnderscore{}window\markdownRendererUnderscore{}quota decision table:\markdownRendererInterblockSeparator
{}\markdownRendererUlBegin
\markdownRendererUlItem Default is 15.\markdownRendererUlItemEnd 
\markdownRendererUlItem Use 20 when coverage.enabled=true and timeline\markdownRendererUnderscore{}mode.enabled=false.\markdownRendererUlItemEnd 
\markdownRendererUlItem Use 25 when timeline\markdownRendererUnderscore{}mode.enabled=true and time\markdownRendererUnderscore{}window.enabled=true only if the time window is narrower than a full day.\markdownRendererUlItemEnd 
\markdownRendererUlItem Use 25 for explicit claim-verification questions with a date/time anchor.\linebreak
{}This includes questions asking whether a statement was true, accurate, supported by evidence, contradicted by records, or what actually happened.\linebreak
{}These questions need same-window corroborating and contradicting events, not just semantically similar older events.\markdownRendererUlItemEnd 
\markdownRendererUlItem Use 25 for narrow activity/session windows when the question asks what happened during a conversation, dinner, movie night, board game session, yoga session, appointment, commute, clinic visit, or practice.\linebreak
{}The answer often depends on several adjacent snippets inside that session.\markdownRendererUlItemEnd 
\markdownRendererUlItem For full-day/date-only windows such as a named weekday, an explicit calendar date, "that day", or 00:00:00-23:59:59, do not let the time window crowd out semantic/BM25 seeds:\markdownRendererInterblockSeparator
{}\markdownRendererUlBegin
\markdownRendererUlItem Use 15 for full-day timeline, full-day reconstruction, complete sequence, throughout-the-day progression, or multi-person/multi-device coverage.\markdownRendererUlItemEnd 
\markdownRendererUlItem Use 10-12 for full-day questions about a specific subject, object, appointment, decision, purchase, message, or incident.\markdownRendererUlItemEnd 
\markdownRendererUlItem Use 20 only when the question explicitly asks for all events across the whole day and lexical anchors are weak.\markdownRendererUlItemEnd 
\markdownRendererUlEnd \markdownRendererUlItemEnd 
\markdownRendererUlItem Do not go below 15 unless there is no time\markdownRendererUnderscore{}window.\markdownRendererUlItemEnd 
\markdownRendererUlItem Never use a full-day quota merely because a calendar date is present.\linebreak
{}First decide whether the question has a narrower activity/session anchor.\linebreak
{}If it does, use the narrower window and its normal quota.\markdownRendererUlItemEnd 
\markdownRendererUlEnd \markdownRendererUlItemEnd 
\markdownRendererUlItem seed.temporal\markdownRendererUnderscore{}neighbor\markdownRendererUnderscore{}keep decision table:\markdownRendererInterblockSeparator
{}\markdownRendererUlBegin
\markdownRendererUlItem Default is 24.\markdownRendererUlItemEnd 
\markdownRendererUlItem When temporal\markdownRendererUnderscore{}neighbors.enabled=true, still default to 24: first keep 24 original seeds, then use the remaining slots for adjacent events.\linebreak
{}Do not go below 24 unless the question clearly requires continuous adjacent-snippet coverage and original semantic recall is not important.\markdownRendererUlItemEnd 
\markdownRendererUlEnd \markdownRendererUlItemEnd 
\markdownRendererUlItem Control confidence means confidence in the enabled decision: clear enable -> enabled=true and 0.7-1.0; clear disable -> enabled=false and 0.7-1.0; ambiguous -> 0.4-0.5.\markdownRendererUlItemEnd 
\markdownRendererUlItem semantic\markdownRendererUnderscore{}queries should cover different retrieval intents of the question without adding unknown facts.\linebreak
{}Prefer 2-3 queries when the question asks for multi-hop, multi-detail, multi-source, timeline, comparison, or checklist-like evidence.\markdownRendererUlItemEnd 
\markdownRendererUlItem Provide at least one semantic query unless the original question is already very short and cannot be usefully rewritten.\markdownRendererUlItemEnd 
\markdownRendererUlItem keywords must be short terms extracted from the original question for lexical matching within time windows.\linebreak
{}Prefer people, places, devices, objects, actions, numbers, colors, game/activity words, health readings, and state words.\linebreak
{}Do not output long phrases, full sentences, generic words, or negated/intensified compound phrases.\markdownRendererUlItemEnd 
\markdownRendererUlItem entities must be people, places, devices, or objects extracted from the original question. Do not leave it empty when such entities exist.\markdownRendererUlItemEnd 
\markdownRendererUlItem Output JSON only, no markdown.\markdownRendererUlItemEnd 
\markdownRendererUlEnd \markdownRendererDocumentEnd

==> prompt_tex/23fb58df2a77083d8c6c5d4150cb2084.md.tex <==
\markdownRendererDocumentBegin
You are a memory retrieval planner. Output strict JSON only.\linebreak
{}Your task is not to answer the question, but to generate a plan for the retrieval system.\linebreak
{}Do not invent specific facts, people, places, devices, or objects that are not present in the user's question.\linebreak
{}You may paraphrase synonyms, decompose intent, preserve evidence requirements, and normalize time expressions.\linebreak
{}The retrieval system uses semantic vector search, BM25 keyword search, time-window seeds, temporal neighbors, and optional coverage diversification.\linebreak
{}When uncertain, lower confidence. confidence means your confidence in the enabled value, not strategy strength.\markdownRendererDocumentEnd

==> prompt_tex/911c7b22ef8c63aba81f98a459367062.md.tex <==
\markdownRendererDocumentBegin
Current new event:\linebreak
{}ID: \markdownRendererLeftBrace{}chunk\markdownRendererUnderscore{}id\markdownRendererRightBrace{}\linebreak
{}Device: \markdownRendererLeftBrace{}device or '?'\markdownRendererRightBrace{}\linebreak
{}Time: \markdownRendererLeftBrace{}timestamp or '?'\markdownRendererRightBrace{}\linebreak
{}Content: \markdownRendererLeftBrace{}event\markdownRendererUnderscore{}text\markdownRendererRightBrace{}\markdownRendererInterblockSeparator
{}Candidate memories:\linebreak
{}\markdownRendererLeftBrace{}\markdownRendererUnderscore{}format\markdownRendererUnderscore{}agent\markdownRendererUnderscore{}candidate\markdownRendererUnderscore{}sections(candidates, max\markdownRendererUnderscore{}fused\markdownRendererUnderscore{}pack\markdownRendererUnderscore{}members=max\markdownRendererUnderscore{}fused\markdownRendererUnderscore{}pack\markdownRendererUnderscore{}members)\markdownRendererRightBrace{}\markdownRendererInterblockSeparator
{}Fused pack capacity:\linebreak
{}Maximum members per fused pack: \markdownRendererLeftBrace{}max\markdownRendererUnderscore{}fused\markdownRendererUnderscore{}pack\markdownRendererUnderscore{}members\markdownRendererRightBrace{}\linebreak
{}Candidate fused nodes at this count are considered full.\linebreak
{}Maximum members removable in one remove\markdownRendererUnderscore{}member operation: \markdownRendererLeftBrace{}max\markdownRendererUnderscore{}remove\markdownRendererUnderscore{}members\markdownRendererRightBrace{}\linebreak
{}If more removals are needed, this pack is not suitable for this event; use create\markdownRendererUnderscore{}fusion\markdownRendererUnderscore{}node, create\markdownRendererUnderscore{}edge, or no\markdownRendererUnderscore{}op instead.\markdownRendererInterblockSeparator
{}Tool budget:\linebreak
{}Additional search\markdownRendererUnderscore{}memory calls used: \markdownRendererLeftBrace{}searches\markdownRendererUnderscore{}used\markdownRendererRightBrace{}\linebreak
{}Maximum additional search\markdownRendererUnderscore{}memory calls: \markdownRendererLeftBrace{}max\markdownRendererUnderscore{}additional\markdownRendererUnderscore{}searches\markdownRendererRightBrace{}\linebreak
{}get\markdownRendererUnderscore{}pack\markdownRendererUnderscore{}members calls used: \markdownRendererLeftBrace{}sum(1 for item in tool\markdownRendererUnderscore{}history if item.get('tool') == 'get\markdownRendererUnderscore{}pack\markdownRendererUnderscore{}members' and not item.get('cached'))\markdownRendererRightBrace{}\linebreak
{}Maximum get\markdownRendererUnderscore{}pack\markdownRendererUnderscore{}members calls: \markdownRendererLeftBrace{}max\markdownRendererUnderscore{}pack\markdownRendererUnderscore{}member\markdownRendererUnderscore{}lookups\markdownRendererRightBrace{}\linebreak
{}Do not call get\markdownRendererUnderscore{}pack\markdownRendererUnderscore{}members just because a pack is full. Call it only when you need member-level evidence to decide whether to update or repair that specific pack.\linebreak
{}Do not call get\markdownRendererUnderscore{}pack\markdownRendererUnderscore{}members to remove members from singleton packs; singleton packs cannot be repaired with remove\markdownRendererUnderscore{}member.\markdownRendererInterblockSeparator
{}[Optional when a tool has been used]\linebreak
{}Tool history:\markdownRendererInterblockSeparator
{}\markdownRendererUlBegin
\markdownRendererUlItem search\markdownRendererUnderscore{}memory query="\markdownRendererLeftBrace{}query\markdownRendererRightBrace{}" returned \markdownRendererLeftBrace{}count\markdownRendererRightBrace{} candidates\markdownRendererUlItemEnd 
\markdownRendererUlItem get\markdownRendererUnderscore{}pack\markdownRendererUnderscore{}members(\markdownRendererLeftBrace{}fusion\markdownRendererUnderscore{}node\markdownRendererUnderscore{}id\markdownRendererRightBrace{}) returned:\linebreak
{}\markdownRendererLeftBrace{}response\markdownRendererRightBrace{}\markdownRendererUlItemEnd 
\markdownRendererUlItem Previous plan rejected: \markdownRendererLeftBrace{}feedback\markdownRendererRightBrace{}\markdownRendererUlItemEnd 
\markdownRendererUlEnd \markdownRendererInterblockSeparator
{}[Optional after a fused pack has been inspected]\linebreak
{}Inspected pack review requirements:\linebreak
{}Inspected fused nodes: \markdownRendererLeftBrace{}fusion\markdownRendererUnderscore{}node\markdownRendererUnderscore{}ids\markdownRendererRightBrace{}\linebreak
{}Next, submit submit\markdownRendererUnderscore{}fusion\markdownRendererUnderscore{}plan; do not inspect the same pack again.\linebreak
{}If you do not output remove\markdownRendererUnderscore{}member, you confirm all inspected\linebreak
{}pack members belong to the same concrete event segment.\markdownRendererInterblockSeparator
{}[Optional when session context is available]\linebreak
{}Session context:\linebreak
{}\markdownRendererLeftBrace{}session\markdownRendererUnderscore{}context\markdownRendererRightBrace{}\markdownRendererInterblockSeparator
{}Output the next JSON object: call search\markdownRendererUnderscore{}memory, get\markdownRendererUnderscore{}pack\markdownRendererUnderscore{}members,\linebreak
{}or submit\markdownRendererUnderscore{}fusion\markdownRendererUnderscore{}plan.\markdownRendererDocumentEnd

==> prompt_tex/fusion-agent-per-turn-user-prompt.tex <==
\input prompt_tex/911c7b22ef8c63aba81f98a459367062.md.tex\relax

==> prompt_tex/query-planner-system-prompt.tex <==
\input prompt_tex/23fb58df2a77083d8c6c5d4150cb2084.md.tex\relax

==> prompt_tex/query-planner-user-prompt.tex <==
\input prompt_tex/1e74d81e324aff07118fc8082be81f88.md.tex\relax
